Adaptive Autonomy in Human-on-the-Loop Vision-Based Robotics Systems

Computer vision approaches are widely used by autonomous robotic systems to sense the world around them and to guide their decision making as they perform diverse tasks such as collision avoidance, search and rescue, and object manipulation. High accuracy is critical, particularly for Human-on-the-loop (HoTL) systems where decisions are made autonomously by the system, and humans play only a supervisory role. Failures of the vision model can lead to erroneous decisions with potentially life or death consequences. In this paper, we propose a solution based upon adaptive autonomy levels, whereby the system detects loss of reliability of these models and responds by temporarily lowering its own autonomy levels and increasing engagement of the human in the decision-making process. Our solution is applicable for vision-based tasks in which humans have time to react and provide guidance. When implemented, our approach would estimate the reliability of the vision task by considering uncertainty in its model, and by performing covariate analysis to determine when the current operating environment is ill-matched to the model's training data. We provide examples from DroneResponse, in which small Unmanned Aerial Systems are deployed for Emergency Response missions, and show how the vision model's reliability would be used in addition to confidence scores to drive and specify the behavior and adaptation of the system's autonomy. This workshop paper outlines our proposed approach and describes open challenges at the intersection of Computer Vision and Software Engineering for the safe and reliable deployment of vision models in the decision making of autonomous systems.

==> 3_PracticalExample.tex <==
\section{CV-Supported Autonomy}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%
DroneResponse deploys multiple sUAS to support emergency response missions~\cite{DBLP:conf/chi/AgrawalABCFHHTK20,agrawal2020model,DBLP:conf/modre-ws/AgrawalCS20}. It is designed as a HoTL system empowered to make and enact decisions~\cite{fischer2017loop} supported by its onboard CV. Enabling higher degrees of autonomy is particularly important in DroneResponse missions, where multiple sUAS are deployed simultaneously to perform time-constrained search-and-rescue, surveillance, or delivery tasks.

%\begin{figure}[t]
%  \centering
%  \includegraphics[width=1\columnwidth]{figures/Mockup3.pdf} 
%  \caption{The sUAS has detected a victim in the river with high confidence and certainty and has therefore abandoned its previous {\it search} task and autonomously switched to {\it tracking} mode. After the fact, the sUAS requests confirmation from the human operator and stream video to the human rescuers. }
%   \label{fig:rivervictim}
%\end{figure}

\rose{this next paragraph is repeated: text is already in introduction}
\subsection{Human Engagement} Consider the example shown in Figure~\ref{fig:rivervictim} which depicts a scenario in which an sUAS annotates and streams video of a candidate victim and requests feedback from the human operator. In fact, the system can be established with varying degrees of autonomy with respect to the actions taken by the sUAS after it detects a candidate victim. For simplicity's sake, we assume only one sUAS has detected the candidate victim -- in this case with a confidence score of 0.35. At this point, the sUAS can (1) ask the operator what to do (HiTL), (2) independently determine whether to activate a \emph{victim found} alert, abort its own search, transition to \emph{tracking} mode, and inform the operator of its decisions (HoTL), or (3) make that determination based on the perceived reliability of the CV model within the current environment. The third option allows the sUAS to operate independently when and where it is able to do so but to otherwise engage the operator in its decision-making process. 

==> 5_SafetyAssuranceCase.tex <==
\section{Safety Assurance Case}
\label{sec:SAC}
\jch{Will redo.} A Safety Assurance Case (SAC)~\cite{bloomfield2010safety,holloway2008safety} creates a hierarchical organization of goal-oriented or claim-based safety arguments~\cite{Hawkins2013}, each of which is supported by evidence such as test results, formal reviews, or simulations~\cite{Bishop1998}. SACs are therefore a useful and well-established technique for supporting developers, architects, safety analysts, and other project stakeholders as they proactively build, evaluate, and provide evidence for the safety of a system~\cite{chen-assurancecase,UKMinistryofDefence2017, Graydon2017}. SACs can be modeled in various ways; however, the most common approaches are Goal Structuring Notation (GSN) \cite{kelly2004goal} and Claims-Arguments-Evidence notation \cite{Adelard}. In this paper we adopt the GSN approach. 

\begin{figure*}[t]
  \centering
  \includegraphics[width=1\textwidth]{figures/SAC.png} 
  \caption{This Safety Assurance Case systematically argues that the different degrees of autonomy enabled by the system satisfice (i.e., sufficiently satisfy) the safety requirement that the operator is engaged in the decision making process as and when needed. Note: This SAC is for explanatory purposes and not all Claims are yet fully implemented in our system. \jch{Will make it legible when I finish}}
   \label{fig:SAC}
\end{figure*}

Our goal is to assess the safety of the system with respect to the non-functional safety requirement that `The system requests help from the operator whenever the vision model lacks sufficient confidence or is  untrustworthy.' Non-functional requirements (NFRs) ... definition here. Something about the SAC. Unlike a functional requirement which is evaluated using Boolean logic (i.e., it works as specified or not), an NFR is evaluated upon a scale of measure (REFS) and a fuzzy goal. In this case, the fuzziness is introduced through the term `sufficient confidence' and `untrustworthy'. NFRs typically exhibit tradeoffs which need to be carefully balanced in the designed solution. In this case, tradeoffs exist between autonomy (i.e., empowering UAVs to make their own decisions so that they can operate more efficiently) and caution (i.e., asking the supervisor to intervene through making critical decisions). Given that the SAC addresses an NFR, the goal is to demonstrate that safety goals are satisfied with the aim of optimizing the chance that the victim will be detected and rescued.



==> GOOD2REF.tex <==
A study from Georgia shows that dark skinned people are more likely to be hit by autonomous cars (due to training bias)
https://arxiv.org/pdf/1902.11097.pdf


  
